Optimal Surrogate Boundary Selection and Scalability Studies for the Shifted Boundary Method on Octree Meshes

The accurate and efficient simulation of Partial Differential Equations (PDEs) in and around arbitrarily defined geometries is critical for many application domains. Immersed boundary methods (IBMs) alleviate the usually laborious and time-consuming process of creating body-fitted meshes around complex geometry models (described by CAD or other representations, e.g., STL, point clouds), especially when high levels of mesh adaptivity are required. In this work, we advance the field of IBM in the context of the recently developed Shifted Boundary Method (SBM). In the SBM, the location where boundary conditions are enforced is shifted from the actual boundary of the immersed object to a nearby surrogate boundary, and boundary conditions are corrected utilizing Taylor expansions. This approach allows choosing surrogate boundaries that conform to a Cartesian mesh without losing accuracy or stability. Our contributions in this work are as follows: (a) we show that the SBM numerical error can be greatly reduced by an optimal choice of the surrogate boundary, (b) we mathematically prove the optimal convergence of the SBM for this optimal choice of the surrogate boundary, (c) we deploy the SBM on massively parallel octree meshes, including algorithmic advances to handle incomplete octrees, and (d) we showcase the applicability of these approaches with a wide variety of simulations involving complex shapes, sharp corners, and different topologies. Specific emphasis is given to Poisson's equation and the linear elasticity equations.

==> Tikz/3DGeometryTable.tex <==
\begin{table}[h!]
\caption{Information for the objects we use to test SBM performance.({\color{red}{Is this needed ? How is this information helpful? I can refine athe triangles of cube too. }})}
\centering
\begin{tabular}{lrrr}
\toprule 
    Object  &Triangles &Max element area & Min element area\\ 
\midrule
    Eiffel Tower & 162454  &{4.83e-3}        &{1.32e-10}\\
    Stanford Bunny &37098         & {1.75e-4}       &{1.48e-05}\\
    Moai   &37344         &{2.44e-4}       &{3.33e-08}\\  
    Armadillo & 345944   &{4.01e-5}     &{3.68e-12}\\
\bottomrule
    \end{tabular}
\label{tab:GeoInfo}
\end{table}

==> Tikz/ActiveElementTable.tex <==
\begin{table}[t!]
\caption{Number of \Interior and \Intercepted elements (Mesh size = $1/2^8$){\color{red}{Again how is this any useful?}}}
\[
\begin{array}{@{}l*{3}{c}@{}}
\toprule
\text{Object} & \multicolumn{3}{c@{}}{\lambda}\\
    \cmidrule(l){2-4}
    & 0 & 0.5 & 1\\
\midrule
        \csvreader[head to column names, late after line=\\]
        {Figures/ActiveElement.csv}{}{ \text{\name} & \zero & \zeroPfive & \one}

\bottomrule
\end{array}
\]
\label{tab:ActiveElement}

\end{table}


==> Tikz/DiskContour.tex <==
\begin{figure}[t!]
\centering
        \includegraphics[width=0.5\linewidth,trim=50 50 50 50,clip]      {Figures/Contour/DiskContour_0p5.pdf}
\caption{Disk's Solution contour and mesh.\color{red}{Need a better zoom version}}
\label{fig:DiskContour}
\end{figure}

\begin{figure}
\centering
        \includegraphics[width=0.5\linewidth,trim=50 20 50 0,clip]      {Figures/Contour/DiskContour_0p5.pdf}
\caption{Disk's Solution contour and mesh.}
\label{fig:DiskContour}
\end{figure}

==> Tikz/GaussPoint.tex <==
\begin{figure}[h!]
 \centering
\begin{tabular}{cc}
 (a) & (b)
 \\
     \multicolumn{2}{c}{
     \begin{subfigure}[b]{0.9\textwidth}   
             \centering 
             {{\small }}    
 			\includegraphics[width=\linewidth,trim=0 50 0 50,clip]{Figures/Marker/CircleMarker.pdf}
             \label{fig:}
             %  trim={<left> <lower> <right> <upper>}
     \end{subfigure}
     }
 \end{tabular}
 \caption{
 Volume Gauss points: (\textit{a}) Element Marker with Gauss quadrature points for volume integration on $\Tilde{\Omega}$ for weak form computation. (\textit{b}) Element Marker with Gauss quadrature points for post-processing computations on $\Omega$ (error computation).} 
\label{fig:GaussPoint}
\end{figure}

\begin{figure}[h!]
 \centering
\begin{tabular}{ccc}
 (a) & (b) & (c)
 \\

     \multicolumn{2}{c}{
     \begin{subfigure}[b]{0.6\textwidth}   
             \centering 
             {{\small }}    
 			\includegraphics[width=\linewidth,trim=0 55 0 50,clip]{Figures/Marker/CircleMarker.pdf}
             \label{fig:}
             %  trim={<left> <lower> <right> <upper>}
     \end{subfigure}
     }
     &
    \centering 
    {{\small }}
    \includegraphics[width=0.38\linewidth,trim=0 0 0 0,clip]{Figures/Marker/CheckFalseIntercepted.pdf}
    %  trim={<left> <lower> <right> <upper>}

 \end{tabular}
 \caption{
 {\textcolor{red}{This figure needs to redrawn. Last one is not needed. Table needs to be converted to subfigure.}}Element Marker:(\textit{a}) Gauss quadrature points for volume integration on $\Tilde{\Omega}$ for weak form computation. (\textit{b}) Gauss quadrature points for post-processing computations on $\Omega$ (error computation).{\color{red}{Not needed here. Will put it at desired place once the paper in complete. Figure is too crowded (\textit{c}) Checking \FalseIntercepted{} elements using $\lambda = 0.5$}}}
\label{fig:GaussPoint}
\end{figure}

\begin{figure}[h!]
        \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\linewidth,trim=0 100 0 100,clip]      {Figures/Marker/IntegrateGPs.png}
        %  trim={<left> <lower> <right> <upper>}
        \caption{Gauss quadrature points for volume integration.}
\end{subfigure}
        \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\linewidth,trim=0 100 0 100,clip]      {Figures/Marker/PostGPs.png}
        \caption{Gauss quadrature points for post-processing computations.}
\end{subfigure}

 \caption{Element Marker:(\textit{a}) Gauss quadrature points for volume integration on $\Tilde{\Omega}$ for weak form computation. (\textit{b}) Gauss quadrature points for post-processing computations on $\Omega$ (error computation).}
\label{fig:GaussPoint}
\end{figure}

==> Tikz/Poisson/DiskContour.tex <==
% \begin{figure}
% \centering
%         \includegraphics[width=0.5\linewidth,trim=50 50 50 50,clip]      {Figures/Contour/DiskContour_0p5.pdf}
% \caption{Disk's Solution contour and mesh.\color{red}{Need a better zoom version}}
% \label{fig:DiskContour}
% \end{figure}

% \begin{figure}
% \centering
%         \includegraphics[width=0.5\linewidth,trim=50 20 50 0,clip]      {Figures/Contour/DiskContour_0p5.pdf}
% \caption{Disk's Solution contour and mesh.}
% \label{fig:DiskContour}
% \end{figure}

==> Tikz/Poisson/Ring.tex <==
% \begin{figure}
%         \begin{subfigure}{0.5\textwidth}
%         \includegraphics[width=\linewidth,trim=0 0 0 0,clip]      {Figures/Contour/RingContour_0p5.png}
%         \caption{Solution contour}
% \end{subfigure}
%         \begin{subfigure}{0.45\textwidth}
%             \begin{tikzpicture}  
%             \begin{axis}  
%             [  
%                 ybar,  
%                 enlargelimits=0.15,  
%                 ylabel={${L_2(\Omega)}$}, 
%                 % xlabel={},  
%                 symbolic x coords={$\lambda = 0$, $\lambda = 0.5$, $\lambda = 1$}, % these are the specification of coordinates on the x-axis.  
%                 xtick=data,  
%                  % nodes near coords, % this command is used to mention the y-axis points on the top of the particular bar.  
%                 nodes near coords align={vertical},  
%                 ]  
%             \addplot coordinates {($\lambda = 0$,0.000173908) ($\lambda = 0.5$,7.48E-05) ($\lambda = 1$,0.000502657)};  
%              \end{axis}  
%             \end{tikzpicture}  
%       \caption{${L_2(\Omega)}$ at mesh size = $\frac{1}{2^7}$}
% \end{subfigure}
% \caption{Solving Poisson Equation on a Ring using SBM}
% \label{fig:Ring}
% \end{figure}

\begin{figure}
        \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\linewidth,trim=0 0 0 0,clip]      {Figures/Contour/RingContour_0p5.png}
        \caption{Solution contour}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \begin{tikzpicture}       
        \begin{axis}[
            % log basis x=10,
            % log ticks with fixed point,
            width = \linewidth,
            % height = \linewidth,
            ybar,
            % y dir=reverse,
             % ymin=50, ymax=800,
            xtick= {0,1,2,3,4,5},
            xticklabels={$1/2^5$,$1/2^6$,$1/2^7$,$1/2^8$,$1/2^9$,$1/2^{10}$},
            bar width=5,
            % ytick={50,100,200,400,800},
    %        xtickla50,bels={$10^2$, $10^3$, $n$},
    xlabel = {$h$},
    ylabel = {$L_{2\lambda}$},
    legend style={at={(0.5,-0.25)},anchor=north, nodes={scale=0.65, transform shape}}, legend columns=3,
    % cycle list/Set1,
    % 	% combine it with 'mark list*':
    % 	cycle multiindex* list={
    % 		mark list*\nextlist
    % 		Set1\nextlist
    % 	}
            ]
    
    \addplot
     +[]
    	table[x expr=\coordindex,y expr={\thisrow{NormalizedError_1p0_adaptive}/\thisrow{NormalizedError_1p0_adaptive}},col sep=comma]{Figures/L2error/L2error2DringOpt.txt};
     
    \addplot
     +[]
    	table[x expr=\coordindex,y expr={\thisrow{NormalizedError_0p0_adaptive}/\thisrow{NormalizedError_1p0_adaptive}},col sep=comma]{Figures/L2error/L2error2DringOpt.txt};
     
    	\addplot
     +[]
    	table[x expr=\coordindex,y expr={\thisrow{NormalizedError_0p5_adaptive}/\thisrow{NormalizedError_1p0_adaptive}},col sep=comma]{Figures/L2error/L2error2DringOpt.txt};
    	% \addplot
     % +[]
    	% table[x expr=\coordindex,y expr={\thisrow{Forward} + \thisrow{Backward}},col sep=space]{Data/WeakScaling/TensorPartitionChannelVariation.txt};
    
    	\legend{$\lambda=1$,$\lambda=0$,$\lambda=0.5$}
       \end{axis}
    \end{tikzpicture}
    \caption{Improvement in $L_2$ error }
\end{subfigure}
\caption{Solving Poisson Equation on a ring using SBM}
\label{fig:Ring}
\end{figure}

==> Tikz/Poisson/star.tex <==
% \begin{figure}[h!]
% \centering
% \begin{tabular}[t]{ C{7.0cm} C{7.0cm}  }
%  (a) & (b)
% \\
%     \begin{subfigure}[b]{0.45\textwidth}   
%             \centering 
%             {{\small }}    			\includegraphics[width=\linewidth,trim=0 0 0 0,clip]      {Figures/Contour/StarContour_0p5.png}
%         %  trim={<left> <lower> <right> <upper>}

%     \end{subfigure}	
%     &
%         \begin{tikzpicture}
%      \begin{loglogaxis}[width=0.4\linewidth, scaled y ticks=true,xlabel={Element size, h},ylabel={${L_2(\Omega)}$},legend entries={$\lambda = 0$, $\lambda = 0.5$, $\lambda = 1$, $slope = 2$},
%      	legend style={at={(0.5,-0.25)},anchor=north, nodes={scale=0.65, transform shape}}, 
%      	%legend pos=outer south, 
%      	legend columns=3,
%      	%title={\footnotesize(b)}, 
%      	xmin=1E-3,xmax=0.1	,cycle list name=mycolorlist]
%      	\addplot table [x={h},y={L2_0p0_adaptive},col sep=comma] {Figures/L2error/L2error2DstarOpt.csv};
%      	\addplot table [x={h},y={L2_0p5_adaptive},col sep=comma] {Figures/L2error/L2error2DstarOpt.csv};
%      	\addplot table [x={h},y={L2_1p0_adaptive},col sep=comma] {Figures/L2error/L2error2DstarOpt.csv};
%         %slope = 2
%      	\addplot +[mark=none, red, dashed] [domain=1e-4:1]{2*x^2};
%      	\end{loglogaxis}
%      	\end{tikzpicture}
% \\
% \end{tabular}
% \caption{Solving Poisson Equation on a star using SBM: (\textit{a}) The solution contour (Mesh size = 0.00195). (\textit{b}) $L_2$ error convergence} 
% \label{fig:3Dcase}
% \end{figure}

% \begin{figure}
%         \begin{subfigure}{0.45\textwidth}
%         \includegraphics[width=\linewidth,trim=0 0 0 0,clip]      {Figures/Contour/StarContour_0p5.png}
%         \caption{Solution contour}
% \end{subfigure}
%         \begin{subfigure}{0.45\textwidth}
%          \begin{tikzpicture}
%      \begin{loglogaxis}[width=\linewidth, scaled y ticks=true,xlabel={Element size, h},ylabel={${L_2(\Omega)}$},legend entries={$\lambda = 0$, $\lambda = 0.5$, $\lambda = 1$, $slope = 2$},
%      	legend style={at={(0.5,-0.25)},anchor=north, nodes={scale=0.65, transform shape}}, 
%      	%legend pos=outer south, 
%      	legend columns=4,
%      	%title={\footnotesize(b)}, 
%      	xmin=1E-3,xmax=0.1	,
%       % cycle list name=mycolorlist
%       ]
%      	\addplot table [x={h},y={L2_0p0_adaptive},col sep=comma] {Figures/L2error/L2error2DstarOpt.csv};
%      	\addplot table [x={h},y={L2_0p5_adaptive},col sep=comma] {Figures/L2error/L2error2DstarOpt.csv};
%      	\addplot table [x={h},y={L2_1p0_adaptive},col sep=comma] {Figures/L2error/L2error2DstarOpt.csv};
%         %slope = 2
%      	\addplot +[mark=none, red, dashed] [domain=1e-4:1]{2*x^2};
%      	\end{loglogaxis}
%      	\end{tikzpicture}
%       \caption{$L_2$ convergence}
% \end{subfigure}
% \caption{Solving Poisson Equation on a star using SBM}

% \end{figure}

% \begin{figure}
%         \begin{subfigure}{0.5\textwidth}
%         \includegraphics[width=\linewidth,trim=0 0 0 0,clip]      {Figures/Contour/StarContour_0p5.png}
%         \caption{Solution contour}
% \end{subfigure}
%         \begin{subfigure}{0.45\textwidth}
%             \begin{tikzpicture}  
%             \begin{axis}  
%             [  
%                 ybar,  
%                 enlargelimits=0.15,  
%                 ylabel={${L_2(\Omega)}$}, 
%                 % xlabel={},  
%                 symbolic x coords={$\lambda = 0$, $\lambda = 0.5$, $\lambda = 1$}, % these are the specification of coordinates on the x-axis.  
%                 xtick=data,  
%                  % nodes near coords, % this command is used to mention the y-axis points on the top of the particular bar.  
%                 nodes near coords align={vertical},  
%                 ]  
%             \addplot coordinates {($\lambda = 0$,0.000418645) ($\lambda = 0.5$,0.000190305) ($\lambda = 1$,0.00033421)};  
%              \end{axis}  
%             \end{tikzpicture}  
%       \caption{${L_2(\Omega)}$ at mesh size = $\frac{1}{2^7}$}
% \end{subfigure}
% \caption{Solving Poisson Equation on a Ring using SBM}
% \label{fig:star}
% \end{figure}

\begin{figure}
        \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\linewidth,trim=0 0 0 0,clip]      {Figures/Contour/StarContour_0p5.pdf}
        \caption{Solution contour and mesh}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \begin{tikzpicture}       
        \begin{axis}[
            % log basis x=10,
            % log ticks with fixed point,
            width = \linewidth,
            % height = \linewidth,
            ybar,
            % y dir=reverse,
             % ymin=50, ymax=800,
            xtick= {0,1,2,3,4},
            xticklabels={$2.4/2^6$,$2.4/2^7$,$2.4/2^8$,$2.4/2^9$,$2.4/2^{10}$},
            bar width=5,
            % ytick={50,100,200,400,800},
    %        xtickla50,bels={$10^2$, $10^3$, $n$},
    xlabel = {$h$},
    ylabel = {$L_{2\lambda}$},
    legend style={at={(0.5,-0.25)},anchor=north, nodes={scale=0.65, transform shape}}, legend columns=3,
    % cycle list/Set1,
    % 	% combine it with 'mark list*':
    % 	cycle multiindex* list={
    % 		mark list*\nextlist
    % 		Set1\nextlist
    % 	}
            ]
    
    \addplot
     +[]
    	table[x expr=\coordindex,y expr={\thisrow{NormalizedError_1p0_adaptive}/\thisrow{NormalizedError_1p0_adaptive}},col sep=comma]{Figures/L2error/L2error2DstarOpt.txt};
     
    \addplot
     +[]
    	table[x expr=\coordindex,y expr={\thisrow{NormalizedError_0p0_adaptive}/\thisrow{NormalizedError_1p0_adaptive}},col sep=comma]{Figures/L2error/L2error2DstarOpt.txt};
     
    	\addplot
     +[]
    	table[x expr=\coordindex,y expr={\thisrow{NormalizedError_0p5_adaptive}/\thisrow{NormalizedError_1p0_adaptive}},col sep=comma]{Figures/L2error/L2error2DstarOpt.txt};
    	% \addplot
     % +[]
    	% table[x expr=\coordindex,y expr={\thisrow{Forward} + \thisrow{Backward}},col sep=space]{Data/WeakScaling/TensorPartitionChannelVariation.txt};
    
    	\legend{$\lambda=1$,$\lambda=0$,$\lambda=0.5$}
       \end{axis}
    \end{tikzpicture}
    \caption{Improvement in $L_2$ error }
\end{subfigure}
\caption{Solving Poisson Equation on a star using SBM}
\label{fig:star}
\end{figure}

==> Tikz/eiffel.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=1.0\linewidth,trim=300 50 300 30,clip]{Figures/STL/eiffelSTL.png}
        \caption{STL file}
        \label{fig:EiffelSTL}
    \end{subfigure}
    \hspace{0.01\linewidth}
    \begin{subfigure}{0.25\textwidth}
        \centering
        \includegraphics[width=1.0\linewidth,trim=0 0 0 0,clip]     {Figures/Contour/eiffelContour_level10.png}
        \caption{Solution contour}
        \label{fig:EiffelSolution}
    \end{subfigure}
    \hspace{0.01\linewidth}
    \begin{subfigure}{0.35\textwidth}
        \begin{tikzpicture}       
        \begin{axis}[
            width = \linewidth,
            height = 0.8\linewidth,
            ybar,
            xtick= {0,1,2,3,4,5},
            xticklabels={$1/2^{10}$},
            bar width=0.2,
            xlabel = {\footnotesize $h$},
            ylabel = {\footnotesize $L_{2\lambda}$},
            legend style={at={(0.5,1.25)},anchor=north, nodes={scale=0.65, transform shape}},
            legend columns=3,
            ]
    
    \addplot
     +[]
    	table[x expr=\coordindex,y expr={\thisrow{NormalizedError_1p0_adaptive}/\thisrow{NormalizedError_1p0_adaptive}},col sep=comma]{Figures/L2error/L2error3DeiffelOpt.txt};
     
    \addplot
     +[]
    	table[x expr=\coordindex,y expr={\thisrow{NormalizedError_0p0_adaptive}/\thisrow{NormalizedError_1p0_adaptive}},col sep=comma]{Figures/L2error/L2error3DeiffelOpt.txt};
     
    \addplot
     +[]
    	table[x expr=\coordindex,y expr={\thisrow{NormalizedError_0p5_adaptive}/\thisrow{NormalizedError_1p0_adaptive}},col sep=comma]{Figures/L2error/L2error3DeiffelOpt.txt};
    	\legend{$\lambda=1$,$\lambda=0$,$\lambda=0.5$}
       \end{axis}
    \end{tikzpicture}
    \caption{Improvement in $L_2$ error }
    \label{fig:EiffelL2}
\end{subfigure}
\caption{Solving Poisson's equation on the Eiffel tower model using SBM:(\textit{a}) The STL file of the Eiffel tower immersed into the background mesh and the bounding box. (\textit{b}) Solution contour of Eiffel Tower with mesh size equal to $1/2^{10}$. (\textit{c}) Improvement plot of $L_{2\lambda}$ and the results show that the optimal surrogate boundary can reduce the $L_{2N}$ error.}
\label{fig:EiffelTower}
\end{figure}
